Predicting Onset of Dementia in Parkinson's Disease Patients

Alzheimer's disease (AD) and Parkinson's disease (PD) are the two most common neurodegenerative disorders in humans. Because a significant percentage of patients have clinical and pathological features of both diseases, it has been hypothesized that the patho-cascades of the two diseases overlap. Despite this evidence, these two diseases are rarely studied in a joint manner. In this paper, we utilize clinical, imaging, genetic, and biospecimen features to cluster AD and PD patients into the same feature space. By training a machine learning classifier on the combined feature space, we predict the disease stage of patients two years after their baseline visits. We observed a considerable improvement in the prediction accuracy of Parkinson's dementia patients due to combined training on Alzheimer's and Parkinson's patients, thereby affirming the claim that these two diseases can be jointly studied.

==> sections/6-scratchpad.tex <==
\begin{comment}

\begin{abstract}
  Alzheimer's disease (AD) and Parkinson's disease (PD) are the two most common neurodegenerative disorders in humans. Because a significant percentage of patients have clinical and pathological features of both diseases, it has been hypothesized that the patho-cascades of the two diseases overlap. Despite this evidence, these two diseases are rarely studied in a joint manner. In this paper, we utilize clinical, imaging, genetic, and biospecimen features to reduce AD and PD patients into the same feature space. By training a machine learning classifier on the combined feature space, we predicted the disease stage of patients two years after their baseline visits. We observed a considerable improvement in the prediction accuracy of Parkinson's dementia patients due to combined training on Alzheimer's and Parkinson's patients, thereby affirming the claim that these two diseases can be jointly studied.

\end{abstract}


%%% Review
\section{Introduction}

Alzheimer’s disease (AD) is an irreversible, progressive neurological brain disease that gradually deteriorates memory and cognitive skills~\cite{Irvine2008}. Age is the predominant known risk factor, with minimum direct relation to sex or race. However, since women tend to live longer than men, they are at higher risk of the disease. Parkinson's disease (PD) is an irreversible, progressive neurological disease that impairs movement. In addition to the hallmark motor symptoms of bradykinesia, tremor, and rigidity, most PD patients develop cognitive impairment (CI), with up to 83\% progressing to dementia. PD patients who progress to dementia (PDD) have reduced quality of life and independence, which adds to the cost of care and results in additional stress for families and caregivers.

% pathological similarities
AD is characterized by progressive impairment in memory, judgment, language, and orientation to physical surroundings. The primary pathological features of AD are neuronal loss and the accumulation of extracellular plaques containing amyloid $\beta$ (A$\beta$) and neurofibrillary tangles (NFT) containing tau. PD manifests as a movement disorder and a distinct form of cognitive impairment with typical pathological characteristics of the accumulation of $\alpha$-synuclein in multiple brain regions. Although AD and PD are clinically distinct entities, the two diseases appear to be closely associated in pathological evidence. A$\beta$, an important hallmark of AD pathology, has also been reported to be present in patients with PD \cite{kempster2010relationships}. Similarly, PD pathologies have also been reported in AD cases. For example, there has been pathological evidence that indicates that Lewy body deposition also exist in AD cases \cite{compta2011lewy}.

% genetic similarities
AD and PD may also share an overlapping genetic background, such as the APOE and MAPT genes, which have been reported to be linked to the presence of A$\beta$ aggregates \cite{polvikoski1995apolipoprotein} and increased tau protein expression. Noticeably, genetic variants of these two genes have also been verified to increase PD risk. These studies indicate a possible pathological overlap and hereditary associations between AD and PD. 

% novelty of our work
% pathological data
% ADD MORE
The notion of AD and PD sharing features has existed for several years, but with minimal research outcomes. For example, a study showed that two genes controlling low-density lipoprotein are associated with a high risk of both Alzheimer's and Parkinson's disease ~\cite{benn2017low}. In addition, previously reported biochemical correlates of cognitive decline in PD include lower levels of cerebrospinal fluid (CSF) amyloid beta, specifically the disease-implicated form of amyloid beta known as ABeta42, and lower levels of plasma epidermal growth factor (EGF), while higher levels of CSF total tau (t-tau) and phosphorylated tau (p-tau) are associated with poorer cognition in Alzheimer's disease \cite{shaw2009cerebrospinal}. Finally, many imaging-based measures have been reported to be associated with cognitive performance in PD. A baseline AD pattern of brain atrophy, quantified using the Spatial Pattern of Atrophy for Recognition of AD (SPARE-AD) score, predicted long-term global cognitive decline in non-demented PD patients \cite{weintraub2011alzheimer}.

% motivation
Despite these multimodal feature similarities, research groups that study AD and PD remain distinct, resulting in separate sources of data. This motivates an aggregative, data-driven study to explore correlation between the two diseases, which should result in a clearer understanding and possible development of therapeutic targets for both ailments. In this paper, we explore clinical, imaging, genetic, and biospecimen features to reduce AD and PD patients into a common feature space. Successful aggregation allows larger sources of combined data for future studies. Additionally, an aggregative study can serve as a baseline with which to observe future similarities between AD and PD patients. We show the potential of combining AD and PD data in a classification task, in which we predict the disease status of patients two years after the baseline visit. Our method achieves significant performance improvements in the classification accuracy of dementia in PD patients due to training our classifier on the combined AD and PD datasets.


\section{Materials and Methods}

\subsection{Data}

The labels used for our task consist of three classes: Normal cognitive impairment (``Normal CI''), Mild Cognitive Impairment (``MCI''), and ``Dementia''. From the ADNI dataset, control patients were assigned ``Normal CI'', MCI patients were already labeled appropriately, and patients with AD were given the ``Dementia'' label. For the PPMI dataset, patients were assigned ``Normal CI'' if their MoCA scores were greater than 26, ``MCI'' if their MoCA scores were within the interval of $[23, 26]$, and ``Dementia'' if their MoCA scores were less than 23. These labels were assigned for both the diagnosis at baseline and the diagnosis after $24$ months.

\subsection{Alzheimer's Disease}

Data used in the preparation of this article were obtained from the Alzheimer’s Disease Neuroimaging Initiative (ADNI) database (adni.loni.usc.edu). The ADNI was launched in 2003 as a public-private partnership, led by Principal Investigator Michael W. Weiner, MD. The primary goal of ADNI has been to test whether serial magnetic resonance imaging (MRI), positron emission tomography (PET), other biological markers, and clinical and neuropsychological assessment can be combined to measure the progression of mild cognitive impairment (MCI) and early Alzheimer’s disease (AD). %TODO Number of patients

We selected ADNI-2 participants meeting the criteria for single-domain or multidomain amnestic MCI, as in prior work \cite{mathotaarachchi2017identifying}. The eligibility criteria of MCI were participants with minimental state examination (MMSE) scores equal to or greater than 24, a clinical dementia rating of 0.5, subjective and objective memory loss, normal activities of daily living, and the absence of other neuropsychiatric disorders, including Alzheimer’s disease, at baseline \cite{petersen2002mild}. Also, an important criteria for assembling patients was availability of features to be used for the prediction task. This resulted in a total of \textit{355} AD patients. 

%In order to predict disease progression, we categorized patients into six groups based on their status at baseline and  their 24-month follow-up visit. A patient's condition \textit{progresses} if he or she is diagnosed with Alzheimer's disease in the follow-upvisit, and \textit{does not progress} otherwise.

\subsection{Parkinson's Disease}

Data used in the preparation of this article were obtained from the Parkinson’s Progression Markers Initiative (PPMI) database (www.ppmi-info.org/data). For up-to-date information on the study, visit www.ppmi-info.org. From the PPMI dataset, we utilized Montreal Cognitive Assessment (MoCA) scores~\cite{nasreddine2005montreal}. MoCA is a widely used screening assessment for detecting cognitive impairment. The scores range between 0 and 30, where a score of over 26 is normal, and lower scores indicate higher cognitive impairment. We used MoCA score to label a patient with respect to its cognitive impairment level. A MoCA score $> 26$ means the patient is normal (with respect to Dementia). MoCA score $\in$ [23,26] implies patient has mild cognitive impairment, and MoCA score $< 23$ labels the patient as Dementia. Note that ~\cite{Dalrymple-Alford1717} and ~\cite{Hoops1738} validate our claim of using MoCA scores for labeling cognitive status in PPMI patients. Based on the availability of MoCA scores, and other required features, we were reduced to $142$ PDD patients.



The following section describes our classification task, our feature selection process, and classifier used to accomplish the task.

\subsection{Classification Task}

In this study, we aim to predict a given patient’s cognitive status (Normal CI/MCI/Dementia) after 24 months using his/her baseline features. Since predicting the onset of dementia in PD patients is of high clinical importance, our primary goal is to improve existing state-of-the-art methodologies for this goal. We combine AD and PD patients into a single dataset to accomplish our task. This is feasible because the onset of dementia in PD patients mimics AD pathology.

\begin{table}[h!]
\centering
\caption{Statistical summary of patients with assigned labels.}
\label{tab:1}
\begin{tabular}{ ccccc } 
\hline
Dataset & Baseline Diagnosis & Future Diagnosis & Number of patients \\
\hline
\multirow{6}{4em}{ADNI} & Normal CI & Normal CI & 131\\ 
& Normal CI & MCI & 11\\ 
& Normal CI & Dementia & 2\\
& MCI & MCI & 144\\
& MCI & Dementia & 48\\
& Dementia & Dementia & 19\\
\hline
\multirow{6}{4em}{PPMI} & Normal CI & Normal CI & 75\\ 
& Normal CI & MCI & 35\\ 
& Normal CI & Dementia & 4\\
& MCI & MCI & 20\\
& MCI & Dementia & 7\\
& Dementia & Dementia & 1\\
\hline
\multirow{6}{4em}{Combined} & Normal CI & Normal CI & 206\\ 
& Normal CI & MCI & 46\\ 
& Normal CI & Dementia & 6\\
& MCI & MCI & 164\\
& MCI & Dementia & 55\\
& Dementia & Dementia & 29\\
\hline
\end{tabular}
\end{table}

The labels used for our task consist of three classes: Normal cognitive impairment (``Normal CI''), Mild Cognitive Impairment (``MCI''), and ``Dementia''. From the ADNI dataset, control patients were assigned ``Normal CI'', MCI patients were already labeled appropriately, and patients with AD were given the ``Dementia'' label. For the PPMI dataset, patients were assigned ``Normal CI'' if their MoCA scores were greater than 26, ``MCI'' if their MoCA scores were within the interval of $[23, 26]$, and ``Dementia'' if their MoCA scores were less than 23. These labels were assigned for both the diagnosis at baseline and the diagnosis after $24$ months.

Table ~\ref{tab:1} summarizes the composition of different types of progressing patients used in our prediction task. Note that we are only concerned with disease progression; hence, we do not consider disease reverter cases (patients who improve in disease condition).

\subsection{Feature Selection}
Clinical studies have shown correlations between certain biomarkers with the onset of dementia. For the purpose of this paper, we considered imaging, genetic, and biospecimen features commonly known to drive dementia prediction ~\cite{berlyand2016}. We describe these features in the following subsections.

\subsubsection{Imaging Features}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{image_features_future_diagnosis.png}
\caption{PCA-induced image features of AD and PD patients.}
\label{fig:1}
\end{figure}

To obtain imaging features, we used the FreeSurferV5.1 software, which can analyze and visualize MRIs \cite{fischl2012freesurfer}. We preprocessed PPMI MRIs at the baseline to generate a finite set of imaging features. We used FreeSurferV5.1, as the ADNI repository had used the same version to generate similar image features. This allowed us to map ADNI and PPMI patients into a unified image feature space. We used Principal Component Analysis (PCA) \cite{pearson1901liii} to reduce the feature space to three dimensions. We used these three principal components in our classification model. Fig ~\ref{fig:1} illustrates all data points in our common feature space generated via PCA. Note that each data point is labeled by its cognitive label after $24$ months in addition to its dataset of origin. We observe that data points in the ADNI and PPMI datasets that share common cognitive statuses are in close proximity with one another. This leads us to the inference that as far as cognitive impairment is concerned, image features from AD and PD patients can show similarity.

\subsubsection{Genetic Features}

We selected a single genetic feature, apolipoprotein E4 (ApoE4), which is the largest known genetic risk factor for late-onset sporadic AD in a variety of ethnic groups \cite{corder1993gene, sadigh2012association}. ApoE4 has also been shown to be associated with cognitive decline in Parkinson's disease \cite{aarsland2017cognitive}.

\subsubsection{Biospecimen Features}

For biospecimen features, we selected cerebrospinal fluid (CSF) total tau, phosphorylated tau 181 protein (p-tau181), and CSF A$\beta 42$ levels. Elevated CSF total tau and p-tau181 concentrations have been shown to be associated with neurodegenerative changes in early AD \cite{thomann2009association, shaw2009cerebrospinal}. CSF A$\beta42$ levels have also been shown to play an essenntial role in all forms of AD pathogenesis \cite{younkin1998role}. Each of these biomarkers also has strong prognostic and diagnostic potential in early-stage PD \cite{kang2013association}.

We considered using the CSF alpha-synuclein levels \cite{irwin2017neuropathological}, but this data was unavailable for ADNI-2/GO participants.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth, height=4cm]{feature_baseline.png}
\caption{Feature value ranges for ADNI and PPMI patients.}
\label{fig:2}
\end{figure}

Because each of these features have strong evidence in literature implicating their roles in the onset of dementia in both AD and PD patients, they are apt for use in our prediction task. One can observe overlaps between feature values of ADNI and PPMI patients in Fig ~\ref{fig:2}, suggesting potential for accurate predictions for both kinds of patients, especially PD patients.

\subsection{Classification}
\subsubsection{Input and Output}
Using the features at baseline (gender, three imaging features, ApoE4 genotype, and the three biospecimen features), we trained a classifier to predict a patient's cognitive disease label two years after the baseline. 

\subsubsection{Classifier}
For our classifier, we used the Random Forest classifier with 500 trees and the max features parameter as 0.6. In our preliminary testing, random forest outperformed other commonly used classifiers such as logistic regression, support vector machine, multi-layer perceptronm, etc. This reaffirms our intuition behind using random forests. Random forests are inherently suited for multi-class problems and work well in combination with numerical, categorical features. They can also output the importance of each feature, which provides interpretability to the results.

\subsubsection{5-fold Cross-Validation}
We used 5-fold cross-validation, splitting the folds on AD and PD patients independently, and recombined them for the training to avoid imbalances between the two diseases. Thus, each fold contained equal proportions of AD and PD patients. We report the accuracy, precision, recall, and AUC values.  

\section{Results}

Table~\ref{tab:results} summarizes our results for the aforementioned classifier. We tested multiple cases in which we changed the training and test sets to obtain insightful results. Note that even though we list accuracy as a performance parameter, it was not used as a measure of comparison because it can misinterpret the performance when the sample has imbalanced class probabilities~\cite{mathotaarachchi2017identifying}. 

%%% Results table
\begin{table}[h!]
    \caption{Summary of results}
    \label{tab:results}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
    Training set & Test set & AUC-Dementia & AUC-MCI & AUC-CI & Accuracy & Precision & Recall\\ [0.5ex] 
    \midrule
    ADNI+PPMI & ADNI+PPMI &  0.88 & 0.64 & 0.72 & 0.53 & 0.57 & 0.53\\
    ADNI+PPMI & PPMI  & \textbf{0.95} & 0.53  & 0.62 & 0.57 & 0.33 & 0.36 \\
    ADNI+PPMI & ADNI &  0.91 & 0.68  & 0.77 & 0.52 & 0.55 & 0.53 \\
    PPMI & PPMI &  \textbf{0.61} & 0.42  & 0.65 & 0.48 & 0.27 & 0.32 \\
    ADNI & ADNI &   0.89 & 0.67  & 0.77 & 0.52 & 0.56 & 0.55 \\
    \bottomrule
\end{tabular}}
\end{table}

%%% TODO: filler content

\begin{figure}[th!]
    \begin{subfigure}{0.33\columnwidth}
    \includegraphics[width=\linewidth, height=4cm]{ROC_ap_ap.png} 
    \caption{}
    \label{fig:roc1}
    \end{subfigure}
    \begin{subfigure}{0.33\columnwidth}
    \includegraphics[width=\linewidth, height=4cm]{roc_ap_p.png}
    \caption{}
    \label{fig:roc2}
    \end{subfigure}
    \begin{subfigure}{0.33\columnwidth}
    \includegraphics[width=\linewidth, height=4cm]{roc_ap_a.png}
    \caption{}
    \label{fig:roc3}
    \end{subfigure}
\caption{Receiver Operating Curves (ROC) for three testing scenarios - (a) Train on ADNI and PPMI, Test on ADNI and PPMI, (b) Train on ADNI and PPMI, Test on ADNI, (c) Train on ADNI and PPMI, Test on PPMI}
\label{fig:roc}
\end{figure}


Fig~\ref{fig:roc} presents the Receiver Operating Curves (ROC) for three relevant testing scenarios in Table~\ref{tab:1}. Class $0$ represents Dementia, class $1$ MCI and class $2$ CI.

%%% Comparative analysis
Fig~\ref{fig:roc1} provides the generalized performance of our model.


In Fig~\ref{fig:roc1}, we observe an AUC value of 0.88 for Dementia, which provides generalized performance. 

In Figure 3b, our model’s future diagnosis on PD patients is very accurate (AUC value 95). This result is of utmost importance, since our main goal is predicting the onset of dementia in PD patients. However, we notice considerably lower AUC values for Normal CI and MCI patients in all test cases. 

Figure 3(c) depicts performance on ADNI test set.  
 
Our model provides high AUC values for dementia, beating state-of-the-art models. Based on our results in Table  2, we can assertively say that using a training set of ADNI and PPMI patients significantly beats the performance of models trained on only PPMI patients. This was made possible by both AD and PD patients sharing common pathology for the onset of dementia, and combining both sets increased the size of data set threefold when compared to using only the PPMI dataset.
 
We acknowledge that performance measures other than AUC values are not as high as expected in all test cases.  This could be attributed to small size of the data set (n = 497 patients).  We had to intersect all patient sets per feature, which also reduced the size. One can notice that our set of PPMI patients is quite small. This was mostly due to the absence of MoCA scores of many PPMI patients.


\begin{figure}[h!]
    \begin{subfigure}{0.5\columnwidth}
    \includegraphics[width=\linewidth, height=3cm]{patient_feature_space_without_apoe.png} 
    \caption{Feature space without APOE genotype}
    \label{fig:apoe1}
    \end{subfigure}
    \begin{subfigure}{0.5\columnwidth}
    \includegraphics[width=\linewidth, height=3cm]{clustered_patient_feature_space.png}
    \caption{Feature space with APOE genotype}
    \label{fig:apoe2}
    \end{subfigure}
    \caption{Comparison of feature spaces without and with baseline diagnosis.}
    \label{fig:apoe12}
\end{figure}


% Without/with APOE analysis
Figure 4 illustrates importance of features used in the classifier. PCA\_1, PCA\_2, PCA\_3 encompass image features. They have a combined importance of ~ 46 $\%$, which points to the necessity of imaging features. Abeta-42 has an importance of 17.5 $\%$, which when combined with Total-tau and p-Tau give considerable significance to biospecimen modality. 

Statistically, ApoE Genotype has a small contribution in prediction outcome, which opposes intuition as it has been found to hold large importance when predicting Dementia. When we refer to Figure 5, we are able corroborate aforementioned notion. Figure 5(a) shows patient feature space with ApoE Genotype while Figure 5(b) shows feature space without ApoE Genotype. One can clearly observe that ApoE Genotype acts as a discriminating feature when predicting future diagnosis. Figure 5(a) depicts formation of clusters when using all mentioned features, while in Figure 5(b) data has lower visual segregation, which might make classifier less effective.

\begin{figure}[h!]
\begin{subfigure}{0.5\columnwidth}
\includegraphics[width=\linewidth, height=5cm]{feature_overlap_after_cluster.png} 
\caption{Feature importances without baseline diagnosis.}
\label{fig:imp1}
\end{subfigure}
\end{figure}

In Figure 5(a), we also plot center of the clusters. Following the label colors, one can observe the composition of both clusters. The cluster covering the lower left portion of the plot has an almost equal concentration of ADNI and PPMI patients of similar labels (Normal\_CI/MCI/Dementia). 

We plot Figure 6 to further correlate features of those ADNI and PPMI patients.  We observe high percentage of overlap between feature values of patients in the lower cluster, especially Abeta-42 which holds the highest feature importance. This justifies our claim of expecting better results by combining ADNI and PPMI patients.

Although there is a dearth of research in prediction of Dementia in PD patients (PDD), we were able to use Berlyand et.al [3] as baseline for our task. They trained a Logistic Regression classifier on a AD cohort of 210 patients to predict control Vs Dementia patients. They, then, used the trained model to predict control vs Dementia on a PD cohort of 75 patients with considerably lower performance. Note that we differ in our experiments - (1) usage of raw image features processed through Freesurfer and reduced through PCA, (2) usage of both AD and PD patients for training the model and (3) prediction of Normal\_CI/MCI/Dementia patients instead of Normal/Dementia patients. We use (1) as it opens up our model to better extract information from images and does not impose bias unlike SPARE-AD score. Using (2) exposes our model to a larger dataset and (3) provides a more fine-grained outcome.

\section{Conclusions}
This paper makes an attempt at predicting the onset of dementia in patients, with special interest to PD patients. This is a task of high clinical importance. We obtain promising results as compared to the state of the art. We show that using AD patients along with PD patients to build a model to predict the onset of dementia in PD patients is a promising future direction. This also reaffirms our claim that dementia in PD and AD share the same pathology. We believe this can help open up new avenues of research going forward.

For future work, we wish to replicate these results on other AD and PD data sets to corroborate our claim. We would also like to further understand the reasoning behind the low accuracy, precision, and recall scores.


\end{comment}

